TimeMixer++: A General Time Series Pattern Machine for Universal Predictive Analysis

Time series analysis plays a critical role in numerous applications, supporting tasks such as forecasting, classification, anomaly detection, and imputation. In this work, we present the time series pattern machine (TSPM), a model designed to excel in a broad range of time series tasks through powerful representation and pattern extraction capabilities. Traditional time series models often struggle to capture universal patterns, limiting their effectiveness across diverse tasks. To address this, we define multiple scales in the time domain and various resolutions in the frequency domain, employing various mixing strategies to extract intricate, task-adaptive time series patterns. Specifically, we introduce a general-purpose TSPM that processes multi-scale time series using (1) multi-resolution time imaging (MRTI), (2) time image decomposition (TID), (3) multi-scale mixing (MCM), and (4) multi-resolution mixing (MRM) to extract comprehensive temporal patterns. MRTI transforms multi-scale time series into multi-resolution time images, capturing patterns across both temporal and frequency domains. TID leverages dual-axis attention to extract seasonal and trend patterns, while MCM hierarchically aggregates these patterns across scales. MRM adaptively integrates all representations across resolutions. This method achieves state-of-the-art performance across 8 time series analytical tasks, consistently surpassing both general-purpose and task-specific models. Our work marks a promising step toward the next generation of TSPMs, paving the way for further advancements in time series analysis.

==> additional_results.tex <==
% \section{Additional Experiments}
% \label{sec:more_experiments}


% \vspace{-1mm}
% \begin{table}[H]
% \renewcommand\arraystretch{1.2}
% \begin{center}
% \caption{Cross-domain Zero-shot learning results. We follow the same protocol as \citep{zhou2023one} and report results from \citep{liu2024autotimes}. $M4\rightarrow M3$ means training the model on the datasets of M4 and then evaluating
% on M3, and vice versa.}
% \label{tab:zero-shot-cross}
% \vspace{-3mm}
% \resizebox{\columnwidth}{!}{
%   \begin{threeparttable}
%   \begin{small}
% \setlength\tabcolsep{4pt}
% \begin{tabular}{c|cccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Methods}} & \textbf{TimeMixer++} & \textbf{FPT} & \textbf{DLinear} & \textbf{PatchTST} & \textbf{AutoTimes} & \textbf{TimesNet} & \textbf{Nsformer} & \textbf{FEDformer} & \textbf{Informer} & \textbf{Reformer} \\
% % \midrule
%  & \citeyearpar{zhou2023one} & \citeyearpar{zhou2023one} & \citeyearpar{dlinear} & \citeyearpar{patchtst} & \citeyearpar{liu2024autotimes} & \citeyearpar{wu2022timesnet} & \citeyearpar{Liu2022NonstationaryTR} & \citeyearpar{zhou2022fedformer} & \citeyearpar{zhou2021informer} & \citeyearpar{kitaev2020reformer} \\
% \midrule
% $M4 \rightarrow M3$ & \textbf{12.49} & 13.06 & 14.03 & 13.06 & 12.75 & 14.17 & 15.29 & 13.53 & 15.82 & 13.37 \\
% $M3 \rightarrow M4$ & \textbf{12.756} & 13.125 & 15.337 & 13.228 & 13.036 & 14.553 & 14.327 & 15.047 & 19.047 & 14.092 \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{threeparttable}
% }
% \end{center}
% \end{table}
% \vskip -0.1in

% \red{As shown in Table.~\ref{tab:zero-shot-cross}, \method demonstrates the best performance across both tasks, outperforming other methods and showcasing its superior ability to generalize temporal patterns without task-specific training. \method consistently delivers the lowest errors, with improvements ranging from 2\% to 33\% compared to competing methods. }

% \vspace{-2mm}
% \begin{table}[H]
% \renewcommand\arraystretch{1.2}
% \begin{center}
% \caption{Inference time comparison across models on long-term forecasting using ETTm1. The results are reported in milliseconds per iteration (ms/iter). Additional efficiency estimations are provided in Section~\ref{sec:efficiency}.}
% \label{tab:inference-time}
% % \vspace{-3mm}
% \resizebox{\columnwidth}{!}{
%   \begin{threeparttable}
%   \begin{small}
% \setlength\tabcolsep{4pt}
% \begin{tabular}{c|cccccccc}
% \toprule
% \textbf{Methods} & \textbf{TimeMixer++} & \textbf{iTransformer} & \textbf{PatchTST} & \textbf{FEDformer} & \textbf{TimeMixer} & \textbf{TIDE} & \textbf{TimesNet} & \textbf{SCINet} \\
% \midrule
% \textbf{Inference Time} & 90 & 130 & 105 & 240 & 90 & \textbf{85} & 160 & 150 \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{threeparttable}
% }
% \end{center}
% \end{table}
% \vskip -0.1in

% \red{As shown in Table.~\ref{tab:inference-time}, \method demonstrates exceptional inference efficiency compared to baseline models. With an inference speed of 90 ms/iter, \method matches the performance of TiDE and outperforms other models, such as TimesNet (160 ms/iter) and SCINet (150 ms/iter), achieving a speedup of 43.75\% and 40\%, respectively.
% }




% \vspace{-1mm}
% \begin{table}[H]
% \renewcommand\arraystretch{1.2}
% \begin{center}
% \caption{Comparison of MLP-mixing and Attention-mixing on forecasting tasks. Results are reported for Mean Squared Error (MSE) and Mean Absolute Error (MAE).}
% \label{tab:mlp-vs-attention}
% \vspace{2mm}
% \begin{threeparttable}
% \begin{small}
% \setlength\tabcolsep{10pt} % Adjust column spacing
% \begin{tabular}{c|cc|cc}
% \toprule
% \textbf{Method} & \multicolumn{2}{c|}{\textbf{MLP-mixing}} & \multicolumn{2}{c}{\textbf{Attention-mixing}} \\
% Horizon & MSE & MAE & MSE & MAE\\
% \midrule
% 96  & 0.587 & 0.271 & 0.412 & 0.297 \\
% 192 & 0.599 & 0.292 & 0.434 & 0.289 \\
% 336 & 0.627 & 0.346 & 0.452 & 0.297 \\
% 720 & 0.641 & 0.377 & 0.483 & 0.311 \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{threeparttable}
% \end{center}
% \end{table}
% \vskip -0.1in


% \red{We evaluated two channel mixing strategies, MLP-mixing and attention-mixing, on the Traffic dataset, which comprises 862 channels. The input context length is fixed at 96, and the prediction horizons are set to \{96, 192, 336, 720\}. From the table, we observe that attention-mixing consistently outperforms MLP-mixing in terms of MSE for all prediction horizons. For example, at the 96-step prediction horizon, attention-mixing achieves an MSE of 0.412, which is a 29.8\% improvement over MLP-mixing. Similarly, at the 720-step horizon, the MSE reduction with attention-mixing is 24.6\%.
% }
